SHOT: Suppressing the Hessian along the Optimization Trajectory for Gradient-Based Meta-Learning

In this paper, we hypothesize that gradient-based meta-learning (GBML) implicitly suppresses the Hessian along the optimization trajectory in the inner loop. Based on this hypothesis, we introduce an algorithm called SHOT (Suppressing the Hessian along the Optimization Trajectory) that minimizes the distance between the parameters of the target and reference models to suppress the Hessian in the inner loop. Despite dealing with high-order terms, SHOT does not increase the computational complexity of the baseline model much. It is agnostic to both the algorithm and architecture used in GBML, making it highly versatile and applicable to any GBML baseline. To validate the effectiveness of SHOT, we conduct empirical tests on standard few-shot learning tasks and qualitatively analyze its dynamics. We confirm our hypothesis empirically and demonstrate that SHOT outperforms the corresponding baseline. Code is available at: https://github.com/JunHoo-Lee/SHOT

==> text/1_introduction.tex <==
\section{Introduction}

With the advent of \textit{deep learning revolution} in the 2010s, machine learning
has widened its application to many areas and outperformed humans in some areas. Nevertheless,
machines are still far behind humans in the ability to learn by themselves, in that humans
can learn concepts of new data with only a few samples, while machines cannot. Meta-Learning
deals with this problem of \textit{learning to learn.}
An approach to address this issue is the metric-based methods 
\cite{simsiam,Protonet,sigmease,BYOL,SimCLR,RelationNetwork,CLIP}, which aims to learn
`good` kernels in order to project given data into a well-defined feature space. 
Another popular line of research is optimization-based methods 
\cite{maml,lstmmeta, LEO}, so-called Gradient-Based Meta-Learning (GBML), which aims
to achieve the goal of meta-learning by gradient descent.

As the most representative GBML methods applicable to any model trained with the gradient
descent process, model-agnostic meta-learning (MAML) \cite{maml} and its variations
\cite{anil,BOIL,leometa} exploit nested loops to find a good meta-initialization point
from which new tasks can be quickly optimized. To do so, it divides the problem into
two loops: the inner loop (task-specific loop) and the outer loop (meta loop). The
former tests the meta-learning property of fast learning, and the latter moves the
meta-initialization point by observing the dynamics of the inner loop. The general
training is performed by alternating the two loops. In this paper, by focusing on the inner loop of GBML
 methods, we propose a new loss term for the outer loop optimization.

To properly evaluate the meta-learning property in the inner loop, GBML samples a new
problem for each inner loop. Fig.~\ref{fig:innerloop} shows how the problem is 
formulated. For every inner loop, the task is sampled from the task distribution. The
classes constituting each task are randomly sampled, and the configuration order 
(class order) is also randomized. This means that the model tackles an entirely new task
at the beginning of each inner loop. Since the task is unknown and the model has to
solve the problem within a few gradient steps (some extreme algorithms \cite{anil,BOIL}
solve the problem in one gradient step), the model typically exploits large learning
rates to adapt quickly. For example, MAML \cite{maml} and ANIL \cite{anil} use significantly 
larger learning rates of 0.4 and 0.5 respectively, for the inner loop compared to that of the outer loop ($10^{-3}$). These rates are much larger than 
those used in modern deep learning techniques such as ViT \cite{VIT}, which 
typically use rates in the order of $10^{-6}$. However, using such large learning 
rates can lead to instability due to high-order terms like the Hessian 
\cite{lecun2015deep}. The issue of instability caused by high-order terms is 
particularly evident during the initial training phase. To 
mitigate this problem, some deep-learning methodologies employ a heuristic 
that utilizes a smaller learning rate at the beginning \cite{VIT,warmup}. 
Given that GBML goes through only several optimizations in the entire inner 
loop, GBML's inner loop corresponds to the initial training phase. Therefore, 
we anticipate that the problem caused by high-order terms may be severe with a 
large learning rate in each inner loop. However, it is noteworthy that GBML 
appears to perform well despite these potential issues. 
%
% In this paper, we aim to answer the corresponding phenomenon by analysing the inner
% loop of GBML. We observed that the gradient of a GBML model is almost constant within
% an inner loop. This means the model becomes linear after the whole process of few-shot
% learning. Also, we explain intuitively that this kind of phenomenon is the key property
% to solving the implicit risk of a large learning rate in the inner loop. Then, we show
% that the corresponding result makes GBML a variant of metric-based meta learning. Although
% there exist some algorithms exploiting the same observation as ours implicitly \cite{reptile,maml},
% to the best of our knowledge, we are the first to explicitly quantify linearity of
% the inner loop and investigate the connection between the GBML model with linearity
% in the inner loop and the metric-based meta learning.
%


In this paper, we investigate the inner loop of GBML and its relationship with the
implicit risk of using a large learning rate with a few optimization steps in the inner loop. 
We observe that the gradient of a GBML model remains relatively constant within 
an inner loop, indicating that the Hessian along the optimization trajectory 
has a minimal impact on the model's dynamics as learning progresses. We hypothesize that this phenomenon is a key property 
that enables GBML to mitigate the risk of using a large learning rate in the inner loop.

Our hypothesis that GBML implicitly suppresses the Hessian along the optimization trajectory suggests
a desirable property for a GBML algorithm. By explicitly enforcing this property instead of relying on implicit suppression, we anticipate that the model will achieve faster convergence and superior performance.
However, enforcing this property is not trivial as it involves dealing with high-order
terms, which naturally require a significant amount of computation. In this
paper, we propose an algorithm called \textit{Suppressing the Hessian along the
Optimization Trajectory} (SHOT) that suppresses the Hessian in the inner loop by minimizing the distance of the target model from a reference model which is less influenced by the Hessian. Our algorithm can enforce
the Hessian to have desirable properties along the inner loop without much increasing
 the computational complexity of a baseline model. %Thus SHOT can be applied on top of any GBML algorithm.
More specifically, SHOT only requires one additional forward pass without any additional backward pass in general cases.

Our algorithm, SHOT, is agnostic to both the algorithm and architecture used in GBML, 
making it highly versatile and applicable to any GBML baseline. To validate the effectiveness
of SHOT, we conducted empirical tests on standard few-shot learning tasks, including
miniImagenet, tieredImagenet, Cars, and CUB \cite{miniimagenet,tieredimagenet,cars,cub}.
Furthermore, we tested SHOT's cross-domain ability by evaluating its performance on different benchmarks.
Also, SHOT can be applied to one-step or Hessian-free baselines, acting as
a regularizer. Our results demonstrate that SHOT can significantly boost GBML in an algorithm- and architecture-independent
manner. Finally, we analyzed the dynamics of SHOT and confirmed that it behaves
as expected.

\begin{figure}[t]
  \begin{minipage}[c]{0.53\textwidth}
    %\hspace{-7mm}
    \includegraphics[width=\textwidth]{figure/innerloopsetting.pdf}
  \end{minipage}\hfill
  \begin{minipage}[c]{0.46\textwidth}
    \caption{
       For the $i$-th inner loop in meta-learning, the
    task, $\tau_i$, is sampled from the task distribution: $N$ (e.g. 3) classes constituting each task are randomly sampled with a random configuration order, meaning that the model does not have any information before it retrieves an unseen task.
    }
    \label{fig:innerloop}
  \end{minipage}
  %\vspace{-3mm}
\end{figure}
%\bibliography{reference}


==> text/2_related_works.tex <==
\section{Related Works}



% Meta Learning is a methodology which aims to learn to learn by itself \citep{metadef1,metadef2}.
% In the meta-learning community, two main lines of researches are actively
% studied: \ie metric-based meta-learning (MBML) and gradient-based meta-learning (GBML). 
% %메타 러닝에 대한 개괄
%Metric-based meta learnin 설명, kernel을 구한다는 것은 뭔지.. 그리고 이것을 어떻게 성취하는지, 최근에 유행하는 Contrastive Learning과 연결하여 설명, 그다음에 FOMAML알고리즘에 이것과 연결했다는 것을 설명


% The core concept of MBML is similar to classic machine learning algorithms such as
% nearest-neighbor classifiers or support vector machines in the sense that it tries
% to learn `good' feature embeddings which can be easily separated by simple algorithms
% or shallow networks \cite{Protonet,BYOL}. Thus, MBML can be interpreted as a methodology
%for learning a `kernel' since its goal is to learn a good encoder. 

% The core concept of MBML is similar to classic machine learning algorithms such as
% nearest-neighbor classifiers or support vector machines in the sense that it tries
% to learn `good' feature embeddings which can be easily separated by simple algorithms
% or shallow networks \cite{Protonet,BYOL}. Thus, MBML can be interpreted as a methodology
% for learning a `kernel' since its goal is to learn a good encoder. To achieve this
% property, one tries to cluster few-shot images of the same class by making a corresponding
% prototype and trains the encoder to make the encoded samples cluster well around the
% prototype \cite{Protonet,liu2020prototype}. Another line of research is self-supervised
% learning \cite{BYOL,SimCLR,simsiam,sigmease}, which scores state-of-the-art performance
% on few-shot learning nowadays. They want an encoder to have the ability to extract general 
% knowledge from the perspective of mutual information. Since their goal is to learn
% a `good' encoder, they usually attach an additional module to the encoder to construct
% an appropriate decision boundary for a given task. 
% %The relationship between our SHOT and MBML is discussed in the Appendix.

GBML, or optimization-based meta-learning, is a type of methodology which wants to mimic
people's rapid learning skill. Thus, a model should learn with a small number of samples 
and gradient steps. To achieve this property, \cite{lstmmeta} tried to save meta-data
to recurrent networks. Recently, MAML-based methods \cite{maml,imaml,leometa,adaptivelr,negativelr} 
are typically considered as a synonym of GBML consisting of nested loops: outer loop
(meta-loop) and inner loop (task-specific loop). They sample few-shot classification
tasks to test the meta-learning property in the inner loop and update the meta-initialization
parameters in the outer loop with SGD. To learn rapidly, they exploit a more-than-thousand
times larger learning rate in the inner loop compared to modern deep learning settings
such as ViT \cite{VIT} and CLIP \cite{CLIP}. Although some researches have proved
their convergence property \cite{metaconvergencehessian, metaconvergencenolr}, they
set infinitesimal size of learning rate to prove convergence. \cite{metaconvergencehessian} 
set the learning rate considering the Hessian \ie setting the learning rate small enough
so that the higher-order terms do not affect the convergence and \cite{metaconvergencenolr}
proved the convergence with the assumption that the learning rate goes to zero. Although
some lines of research have shown algorithms dealing with learning rates \cite{adaptivelr,negativelr},
they did not explain the success of a large learning rate. \cite{adaptivelr} used
an additional model to predict a proper task-specific learning rate. ANIL (Almost No Inner Loop) \cite{anil} and BOIL (Body Only Inner Loop) \cite{BOIL}
tried to explain GBML with the dynamics of the encoder's output features. Although
both used the same feature-level perspective, they argued in exactly different ways. 
ANIL~\cite{anil} argued feature reuse is an essential component, while BOIL~\cite{BOIL} said
that feature adaption is crucial. Both algorithms can be considered as a variant of
preconditioning meta-learning  since they freeze most layers in the inner loop, thereby
frozen layers can be considered as warp-parameters \cite{warpgrad}. Our SHOT 
can be viewed as a variant of preconditioning, as we hypothesize
that there exists a suitable condition of meta-parameter that can adapt well to a given meta-learning 
task. However, unlike previous work, we define the condition of the meta-parameter based on 
the curvature of the loss surface. Additionally, our algorithm does not require any specific architecture
such as warp-parameters, making it applicable to any architecture and any GBML algorithm. \jh{Finally, there exists some paper which delt with curvature, those all required some special architecture \cite{curvature2}, or explicit calculation of the Hessian \cite{curvature3, curvature1}. In contrast, we propose much weaker condition and does not require specific architecture. We only suppress the Hessian along the inner loop.}
% 해당 precondited method들 중에서 우리의 것과 유사하게 curvature를 다루는 논문들이 존재하였만, 그 논문들 모두 이를 해결하기 위하여 특별한 아키텍쳐를 요구하거나 \cite{curvature2} , Hessian을 직접적으로 업데이트 하는 과정을 거쳤다 \cite{curvature1,curvature3} 하지만 우리는 Hessian을 직접 다루는 것보다 훨씬 더 완화된 조건을 사용함으로서 Hessian을 직접적으로 계산하지 않으며, meta learning의 dyanmics의 특이점에 더 적합한 제한 조건을 제시한다.
In addition, we discuss in the Appendix the possibility of integrating the hypotheses proposed in ANIL~\cite{anil} and BOIL~\cite{BOIL} into our SHOT framework. 

Optimization methods based on second-order or first-order derivatives that take curvature into account
is a vast area of research. Although they incur a higher computational cost than vanilla
SGD, they have been demonstrated to exhibit superior convergence properties. Several studies
have investigated the curvature of the loss surface while maintaining the first-order computational
costs. Natural gradient descent \cite{Riemannian}, a type of Riemannian gradient descent employing the
Fisher information metric as a measure, is coordinate-invariant, and exhibits better
convergence properties than vanilla gradient descent. Given that GBML utilizes relatively
fewer samples, incorporating second-order terms is computationally more feasible. As
a result, there is a growing body of research that employs natural gradient descent
in the inner loop. Additionally, the SAM optimizer~\cite{DBLP:journals/corr/abs-2010-01412} implicitly leverages curvature by
iteratively searching for flat minima during training, leading to better generalization
properties than SGD. This means they find a point where the Hessian is close to zero around a local minimum.
\jh{Our method can be interpreted as the variation of Knowledge Distillation \cite{KD1}. We reduced the distance between models, slow model and fast model. However, we do not need any pretrained model. Those models share same meta-initialization parameter.} 
% 우리의 알고리즘에서 Hessian을 줄이는 데 사용한 방식은, less-Hessian-influenced model과 more-Hessian-influenced model간의 거리를 줄이는 방식으로 이루어져 있기 때문에 Knowledge distillation 방식의 일종으로 볼 수 있다 \cite{KD1} 하지만 우리의 방식의 경우 pretrained된 teacher가 있는 것이 아닌, 같은 meta-initializaer를 공유하는 모델이 같은 data query를 가지고 다른 세팅으로 inner loop하는 것 사이의 거리를 줄였기에 차이가 잇다.}

As our goal is to find a proper meta-initialization point that is not affected by the Hessian along the inner loop, our proposed algorithm, SHOT, also deals with the Hessian of the loss surface.
However, unlike SAM optimizer~\cite{DBLP:journals/corr/abs-2010-01412}, we do not seek a point where the Hessian is zero in any direction. We 
rather seek a point where the Hessian does not take effect only along the optimization trajectory in the inner loop. By using
this restriction, we give a looser constraint. Also, while the SAM optimizer has a nested loop to find a proper point, SHOT does not need any iteration in a single optimization step. %SAM optimizer uses \nj{a} nested loop to find a proper point. 
Also, although natural gradient descent regards curvature like our algorithm, our
SHOT does not calculate the exact Hessian during inference time as we precondition the Hessian and 
only consider the Hessian's effect along the optimization trajectory.
  % Our proposed algorithm, also deals with the Hessian of the loss surface.
% Our goal is to find a proper meta-initialization point that doesn't effected by the Hessian along the inner loop.
% However, unlike SAM optimizer~\cite{SAM} we don't seek a point where the Hessian is zero to entire surface. We 
% rather seek a point where the Hessian does not effect only along the optimization trajectory inner loop. By using
% this restriction, we give a loose constraint. Also, it doesn't need any iteration on single optimization step. SAM optimizer
% uses nested loop to find a proper point. Also, although natural gradient descent regards curvature like our algorithm, our
% algorithm doesn't need to calculate the exact Hessian during inference time. As we precondition the Hessian and 
% only consider the Hessian's effect along the optimization trajectory.
%
In this paper, we aim to shed light on how GBML's inner loop works. 
Through an analysis of the curvature of the loss surface in the inner loop, we hypothesize
that the primary role of the outer loop is to implicitly regulate the curvature of the inner
loop's loss surface. To reinforce this property by explicitly incorporating a corresponding loss term in the inner loop, we propose an algorithm called SHOT, which takes
into account the curvature of the loss surface in the inner loop and aims to enhance
its generalization properties and dynamics by controlling the curvature itself. We provide empirical evidence supporting our hypothesis through the success of SHOT. Additionally, we offer a new interpretation of GBML as a variant of MBML in the Appendix.


==> text/3_preliminaries.tex <==
\section{Preliminaries: GBML}
\label{sec:prelim}
\begin{figure}[t]
\centering
  \begin{minipage}[c]{0.3\textwidth}
    %\hspace{-7mm}
    \includegraphics[width=\textwidth]{figure/close_SHOT_cropped.pdf}
  \end{minipage}\hfill
  \begin{minipage}[c]{0.65\textwidth}
    \caption{
      This figure provides the concept of the proposed SHOT. %, including the optimization
      %process in the inner loop. 
      Specifically, a reference model ($\hat{\theta}^\star$) is 
      initialized with the same support set and starting point as our model (${\theta}^\star$),
      but undergoes significantly more optimization steps. The outer loop then minimizes the
      distance between the two models.}
    \label{fig:SHOT}
  \end{minipage}
  %\vspace{-3mm}
\end{figure}
We consider the few-shot classification task of $N$-way $K$-shot, which requires learning
$K$ samples per class to distinguish $N$ classes in each inner loop. In few-shot GBML, we can apply gradient descent for only a limited number of steps for fast adaptation.

Let $f(x|\theta) \in \mathbb{R}^N$ be the output of the classifier parameterized
by $\theta$ for a given input $x$. In this setting, $f(\cdot)$ can be considered as the logit
before the softmax operation. The model parameters $\theta$ are updated by the loss, 
$L(x,y |\theta) = D( s(f(x|\theta)), y)$, where $x$ and $y$ are the input and the
corresponding label, $s(\cdot)$ is the softmax operation and $D(\cdot,\cdot)$ is some
distance metric.

As shown in Fig.~\ref{fig:innerloop}, at each inner loop, we sample a task 
$\tau \sim p(\mathcal{T})$, an $N$-way classification problem consisting of two sets
of labeled data: $\mathcal{X}_{s}^\tau$ (support set) and 
$\mathcal{X}_{t}^\tau $ (target set). In the inner loop, the goal is to find the 
task-specific parameter $\theta^\star_\tau$ which minimizes the loss $L$ for the support 
set $\mathcal{X}_{s}^\tau$ given the initial parameter $\theta_0$ as follows: %
%
\begin{equation}\label{eq:innerloop}
  \text{Inner Loop:} \quad  \theta^\star_\tau = \underset{\theta}{\arg\min} \sum_{(x,y) \in \mathcal{X}_{s}^\tau}L(x, y|\theta;\theta_0).
\end{equation}
%
Normally, $\theta^\star_\tau$ is obtained by SGD \citep{metadef2,LEO,BOIL,anil}: 
%\begin{equation}
$  \theta^{k+1} = \theta^{k} - \alpha\nabla_{\theta}L(\theta^k), $
%\label{eq:iterin}
%\end{equation}    
where $k$ indicates an inner loop optimization step and $\alpha$ is a learning rate.
%\jh{For ease of notation, we notate $\theta^\star_\tau$ as $\theta^T$. Where $T$ is the total number of optimization step. Assuming task-specific 
%parameter is got by gradient descent.}
We use $T$ steps in the inner loop.

Then, for the outer loop, we optimize the initialization parameters $\theta_0$ which
improve the performance of $\theta_\tau^\star$ on $\mathcal{X}_{t}$ as follows:
%
\begin{equation}\label{eq:outerloop}
   \text{Outer Loop:} \quad \theta_0^\star = \underset{\theta_0}{\arg\min} \sum_{\tau} \sum_{(x,y)\in \mathcal{X}_{t}^\tau} L(x,y|\theta^\star_\tau;\theta_0).
\end{equation}
%
Although GBML gained its success with this setting, this success is quite curious:
since $N$ classes constituting each task are randomly sampled and the configuration
(class) order is also random, `What characteristics of meta-initialization $\theta_0$ 
make GBML work?' remains quite uncertain. 

%추가해야 할것, notation 몇 에폭마다.. 이거 추가하자.


==> text/4_SHOT.tex <==
\section{Optimization in GBML}\label{sec:reduce_hessian}
\subsection{Hypothesis: Outer loop implicitly forces inner loop's loss surface linear}
The perspective of gradient flow provides a way to understand the dynamics of optimization.
In this view, the evolution of model parameters is seen as a discretization of continuous
time evolution. Specifically, the equation governing the model parameters is $\dot
{\theta} = -\nabla_{\theta}L(\theta)$, where $\theta$ represents the model parameter and $L(\theta)$ is the loss function. 
With gradient flow, we can characterize our models into two principal types: the \textbf{Fast Model} and the \textbf{Slow Model}. These definitions emerge from our observation of the models' convergence timelines.  \jh{Considering the terminal point in time as 1 and the initialization as 0, we deduce the timestamp of a singular learning step as $\frac{1}{N}$, where N signifies the number of steps.}

\jh{\textbf{Fast Model}: A model with a relatively small value of N is should converge rapidly. A salient exemplar is GBML's inner loop, typically evolving within a minuscule span of 1 to 5 optimization steps. Such rapid convergence necessitates an elevated learning rate.}

\jh{\textbf{Slow Model}: In contrast, models with a larger value of N take longer to converge. Traditional deep learning models fall into this category. They require many gradient steps and a lower learning rate.}

\jh{This separation makes clear the differences between typical deep learning models and GBML's inner loop. However, we should note that GBML's high learning rate approach can arise some issues.}
% \jh{우리는 이러한 과정을 통해서 fast model과 slow model을 정의할 수 있다. 우리는 학습 과정이 끝난 모델을 converged model, 다시 말해서 evolution이 끝난 모델이라고 생각할 수 있는데, 이때의 시간을 1이라고 하고, initialization일때의 시간을 0이라고 하면 한 step에서의 time stamp는 1/N (number of step)이라고 할 수 있게 된다. 이때 N의 숫자가 상대적으로 적은 모델을 fast (converged) model, N의 숫자가 큰 모델을 slow (converged) model이라고 이야기 할 수 있다. 따라서 이때 parameter의 속도는 상대적으로 느릴 필요가 있고, small $\nabla$, 작은 learning rate를 사용한다. 이 관적에서 conventional deep learning 모델의 경우 slow model에 다 해당된다고 할 수 있다 왜냐하면 일반적으로 converge 될 때까지 거의 infinite number of gradient step을 거치기 때문이다. 하지만 GBML의 inner loop로 오게 된다면, GBML의 경우 optimization step이 일반적으로 1 step부터 5 step까지 매우 적은 step만으로 evolve해야 하기 때문에 fast model에 해당한다. 결과적으로 GBML은 이 문제를 해결하기 위해서 large $\nabla$, 매우 큰 learning rate를 사용하게 된다. 하지만 이 경우, 문제가 생긴다.}

\begin{equation}\label{eq:lossdec}
  \int_{0}^{1}\nabla L(\theta(t)) \cdot \nabla L( \theta^k) dt \approx \int_{0}^{1} 
  \|\nabla L(\theta^k)\|^2_2 -\alpha t \nabla L(\theta^k)^T H(\theta^k) \nabla L(\theta^k) dt >0,
\end{equation}

\jh{Gradient descent is the notion of treating the model as a (locally) linear approximation, adjusting its parameters in a direction where the loss decreases most rapidly. If a model adheres to Eq.~\ref{eq:lossdec}, we can expect the gradient descent effective in that context. (Refer to Appendix \ref{Appendix:Proof of Loss Goes down} for the detailed proof.) However, the inner loop of GBML can be characterized as a fast model. This implies a pronounced influence of the Hessian in the optimization dynamics. Due to this, we cannot guarantee loss decreases in the inner loop. In this paper, We argue that the outer loop's primary role in GBML is to counteract this influence of the Hessian. In more specific terms, it aims to attenuate the impact of \(H(\theta^k) \nabla L(\theta^k)\) on the optimization trajectory.}

% \jh{Gradient descent의 본질은 model을 (locally) linear model로 간주하고, 이 상태에서 loss가 가장 빠르게 줄어드는 방법으로 파라미터를 움직인다. 이 경우에 모델은 Eq.~\ref{eq:lossdec}를 만족하게 된다면 gradient descent가 효과적이라고 생각할 수 있는 것이다. (See the Appendix \ref{Appendix:Proof of Loss Goes down} for the proof.)하지만 GBML의 inner loop는 fast model이라고 할 수 있다. 따라서 Hessian의 영향은 매우 커진다. 그렇기 때문에 우리는 매 inner loop에서는 제대로 학습이 진행된다고 장담할 수 없으며, 우리는 outer loop의 역할이 이 과정에서 Hessian을 줄인다고 주장한다. 더 자세하게는, $H(\theta^k) \nabla L(\theta^k)$, 즉 optimizatino trajectory에서 Hessian의 영향을 줄여준다고 주장한다. }

% This approach is suitable for conventional deep
% learning, which involves almost an infinite number of steps. As the time step $\Delta
% t$ approaches an  infinitesimal value, the first-order term of the Taylor expansion
% of the loss function is sufficient to explain the optimization dynamics. However, this
% approach is not applicable to the inner loop of GBML, which involves only a few steps. 
% As a result, the value of $\Delta t$ can not be regarded as infinitesimal. Therefore, the 
% first-order term of the Taylor expansion of the loss function is insufficient to wholly explain
% the dynamics of optimization in GBML. Instead,  the higher-order terms involving the Hessian appear
% in the dynamics of optimization in the inner loop.

%the first-order term of the Taylor expansion of the loss function is insufficient to fully explain the optimization dynamics in GBML. Instead, the higher-order terms involving the Hessian play a crucial role in the optimization dynamics of the inner loop.
%따라서 우flsms Hessian에 대해서 다루어야 ㅎㄴ다. 이때 inner loop에서 Hesssian이
% ㅈ적어도 Gradient Descent가 일어나게, ㄷktl akfgotj loss가 줄어들려면 어떤 조건을 만족해야 하는가? 
% eq. \ref~{}의 표현을 사용ㅎ여 formal하게 써보면 다ㅇmarhk rkxek.
%\textbf{Outer loop implicitly force inner loop's loss surface linear}

% This phenomenon is problematic because gradient descent does not take the Hessian into account. When the Hessian appears in the training dynamics, it can actually hinder Gradient Descent's ability to perform its intended role. In fact, there are cases where gradient descent can actually increase the loss after optimization. In
% the gradient descent setting of $\theta^{k+1} = \theta^k - \alpha \nabla L (\theta^k)$, the loss $L$ decreases if and only if
%
%
% for a path $\theta(t)$ joining $\theta(0) = \theta^k$ and $\theta(1) = \theta^{k+1}$ (See the Appendix \ref{Appendix:Proof of Loss Goes down} for the proof.).
% %\nj{the} model gets better when \nj{the} Hessian meets \nj{the} following condition:

% From Eq.~\ref{eq:lossdec}, we can see that it's important to reduce the Hessian along the trajectory to ensure that the loss is effectively minimized. Specifically, we want $H(\theta^k) \nabla L(\theta^k)$ to be small in magnitude. We claim that the outer loop of the training process deals with this problem and ensures that the condition in Eq.~\ref{eq:lossdec} is met.


% aspect of GBML, where the condition of curvature is more important than in conventional
% \nj{deep learning}. Consequently, GBML should aim to reduce the loss to zero in the inner loop with
% only a few optimization steps, despite being sensitive to the Hessian. From this perspective,
% We can hypothesize that any successful GBML's outer loop should address the Hessian
% in the inner loop. Specifically, the outer loop should ensure that the Hessian meets
% the condition in \nj{Eq.~}\ref{eq:lossdec}.
%

% \begin{wrapfigure}{l}{0.3\textwidth}
%   \begin{center}
%     \includegraphics[width=0.3\textwidth]{figure/cossimallmethod-3.pdf}
%   \end{center}
%   \caption{This figure compares the cosine similarity between the overall parameter difference
%       and each step's gradient over the training epochs. As training progresses, the cosine
%       similarity increases as training progresses, indicating that the gradient does not vary much over the inner
%       loop. The center and right figures show the results of applying SHOT to MAML.}
% \end{wrapfigure}

%Fig. \ref{fig:cosine} supports our hypothesis. As previously mentioned, the optimization steps are a discretized version that allows for a one-to-one correspondence to time and the current total number of optimization steps conducted. This enables us to observe how the gradient changes as time progresses in the initial dynamics. We can divide this into two parts: how the \nj{gradient's} direction and \nj{magnitude} differ. Surprisingly, in meta-learning, the directions and \nj{magnitudes} do not change \nj{much} as time progresses, whereas in conventional deep learning, they change entirely and differ from the initial dynamics.

\begin{figure}[t]
 
    \includegraphics[width=\textwidth]{figure/allfigonce.png}
    \caption{(left) \textbf{Averaged cosine similarity} between the overall parameter difference ($\theta^\star_\tau - \theta_0$)
      and each step's gradient $(\nabla_{\theta^{k}}L(\theta^k))$ in the inner loop  over the training (meta) epochs. The cosine
      similarity increases as training progresses, indicating that the gradient does not vary much during an inner
      loop. (right) %Qualitative analysis of SHOT. We plotted
    %cosine similarity and 
    \textbf{Validation accuracy vs. training epoch}. To ensure a fair
    comparison, we shifted $\text{SHOT}_p$ for 30 epochs as it pretrains for 30 epochs with $L_{SHOT}$ only. For this figure, we trained $\text{SHOT}_r$ for 300 epochs to compare it at a glance. Our results show that SHOT converges much faster than the baseline. Additionally, we observed a strong correlation between
    cosine similarity and validation accuracy.}
    \label{fig:cosine}
  %\vspace{-3mm}
\end{figure}

Fig. \ref{fig:cosine} supports our claim. As mentioned before, the optimization steps are a discrete representation of the gradient over time. This allows us to track how the gradient changes as time progresses. In meta-learning, the gradient's direction and magnitude do not change significantly as time progresses. This is because meta-learning algorithms are designed to learn how to quickly adapt to new tasks. By learning how to adapt to new tasks, meta-learning algorithms can avoid the need to learn from scratch on each new task. In contrast, in conventional deep learning, the gradient's direction and magnitude change significantly as time progresses. This is because conventional deep learning algorithms are not designed to learn how to quickly adapt to new tasks. Instead, conventional deep learning algorithms are designed to learn a general model that can perform well on a wide variety of tasks. The difference in how the gradient changes over time between meta-learning and conventional deep learning is one of the key factors that explains why meta-learning algorithms are able to learn new tasks so quickly.

It seems clear that Eq.~\ref{eq:lossdec} plays a crucial role in GBML, suggesting 
that we can enhance its performance and dynamics by explicitly inducing the model 
to meet this condition. However, the challenge remains: how can we directly reduce 
the Hessian?


\subsection{SHOT (Suppressing Hessian along the Optimization Trajectory)}

In this part, we present our novel algorithm, Suppressing Hessian along the Optimization Trajectory 
 (SHOT), which is the main contribution of our paper. SHOT is designed
to obviate the effect of the Hessian along the inner loop while maintaining the order of computation cost.

As previously discussed, directly reducing the Hessian is impractical. However, we 
can reduce the effect of the Hessian along the optimization trajectory, specifically 
by minimizing the product $H(\theta_t) \nabla L(\theta_t)$, which is in line with 
the condition expressed in Eq.~\ref{eq:lossdec} and computationally
feasible. To achieve this, we define a measure that quantifies the effect of the 
Hessian along the optimization trajectory.

To do so, we first create a reference model that is not influenced 
by the Hessian. We obtain this reference model by increasing the number of optimization 
steps. The intuition behind this is that as we increase the number of optimization 
steps, the smaller the discretized step becomes, which means that the model with 
many optimization steps is less influenced by the Hessian. We then define the measure 
as the distance between the target model (a model with few optimization steps, $\theta_t$) and 
the reference model (a model with many optimization steps, $\theta_r$). This distance metric, 
denoted as $D(\theta_{t}, \theta_{r})$, quantifies the distortion along the optimization 
path and evaluates the deviation from the ideal optimization trajectory. By minimizing 
this measure, we can achieve our goal of reducing the effect of the Hessian along 
the optimization trajectory. We will call this method as SHOT (Suppressing
Hessian along the Optimization Trajectory) which adds the following loss term in the outer loop of a conventional GBML algorithm:
\begin{equation}
  L_{SHOT} = D(\theta_t^T, \theta_r^R).
  %\mathcal{D}(f(x_t|\theta_{t}^T),f(x_t|\theta_{r}^R)) \  \text{where } \  x_t \in \mathcal{X}_{t}^\tau
  %\text{and} \
  %\theta \text{ is optimized through } x_{s} \in \mathcal{X}_{s}^\tau,  
\label{eq:SHOT}
\end{equation}    
Here, $T$ and $R$ denote the number of steps in an inner loop used to obtain the target and reference model respectively.
In this paper, we used KL divergence ($KL(s(f(\theta_t^T))|s(f(\theta_r^R))$) as a distance metric $D$, but we also conducted
experiments with other distance metrics such as $L_2 (||\theta_t^T - \theta_r^R||_2^2)$ and cross-entropy ($-\sum_c s(f(\theta_t^T))_c \log s(f(\theta_r^R))_c$, as shown in
Table. \ref{table:other_distance}. We set $T<R$ because our intention is to measure
distortion caused by the Hessian in the inner loop. As we increase the number of optimization
steps in the inner loop, the effect of distortion by the Hessian decreases. Therefore,
we could use SHOT as a pseudo-measure of distortion in the inner loop caused by the
Hessian. To match the scale of distribution between $\theta_{t}^T$ and $\theta_{r}^R$,
we set $\alpha$ in Eq.~\ref{eq:innerloop} as $\alpha_{r} = \frac{T}{R} \alpha_{t}$.

Reducing the effect of Hessian along the optimization in the inner loop, as measured 
by Eq.~\ref{eq:SHOT}, can lead to faster
convergence and better performance. By minimizing the deviation from
the ideal optimization trajectory, SHOT can effectively enforce the condition expressed
in Eq.~\ref{eq:lossdec}, which is critical for the success of GBML.  As shot is
the measure of distortion in the whole trajectory of an inner loop. We use SHOT at the
outer loop, where \textbf{scoring} of each optimization trajectory is done.

\input{text/table/RandomvsLIL.tex}

Table \ref{table:randomfeature} highlights the importance of distortion in GBML. We compared
the performance of a randomly-initialized model with that of a lower-distortion-initialized
model, where we only reduced the distortion introduced in Eq.~\ref{eq:SHOT} in the outer loop. As our SHOT loss is self-supervisory that can be applied without target class labels, no target labels are given here.
The results demonstrate that the lower-distortion-initialized model outperforms the randomly-initialized
model, indicating that distortion is a crucial factor in GBML. This also suggests that
we can generally improve GBML by incorporating our loss term, SHOT.

%\subsection{SHOT, as a training scheme in outer loop as a regularizer or meta-meta-initializer}
% \begin{algorithm}
% \caption{$\text{SHOT_r}$ Algorithm}
% \begin{algorithmic}[1]
% \State \textbf{Initialize} parameter $\theta$ (the model)
% \While{not reach max number of epochs}
%     \Comment{Sample query set $Q$, support set $S$}
%     \State \textbf{Start of Inner loop}
%     \State \textbf{Initialize} reference model and target model with $\theta$
%     \State $\theta_r, $\theta_t$= \theta, \theta$
    
%     \Comment{Optimize $\theta_r$ with more (e.g. 3) inner loop steps and a smaller learning rate $\alpha$}
%     \For{$i$ in range(3)}
%         \State $\theta_r = \theta_r - \alpha \cdot \text{gradient}(\text{loss}(\theta_r, S), \theta_r)$
%     \EndFor
    
%     \Comment{Optimize $\theta_t$ with less (e.g. 1) inner loop steps and a larger learning rate $3 \cdot \alpha$}
%     \State $\theta_t = \theta_t - 3 \cdot \alpha \cdot \text{gradient}(\text{loss}(\theta_t, S), \theta_t)$
%     \State \textbf{End of Inner loop}
    
%     \State \textbf{Start of Outer loop}
%     \Comment{Calculate outer loss}
%     \State $\text{outer\_loss} = \text{loss}(\theta_r, Q)$
%     \Comment{Reduce the distance between $\theta_r$ and $\theta_t$ using KL-divergence}
%     \State $\text{kl\_loss} = \text{KL\_divergence}(\text{target\_distribution}(\theta_t, Q), \text{reference\_distribution}(\theta_r, Q).\text{detach}())$
%     \State $\text{outer\_loss} += \lambda \cdot \text{kl\_loss}$
%     \Comment{Use meta-optimizer to optimize parameter $\theta$}
%     \State $\theta = \theta - \beta \cdot \text{gradient}(\text{outer\_loss}, \theta)$
%     \State \textbf{End of Outer loop}
% \EndWhile
% \State \textbf{End of training loop}
% \end{algorithmic}
% \end{algorithm}

\subsection{SHOT can be used as a regularizer or meta-meta-initializer in the outer loop.}

One potential approach to incorporating SHOT is to use it as a regularizer in GBML. 
% \jh{\ie adding SHOT to the loss function of the outer loop during training.}
This approach involves adding SHOT to the loss function
of the outer loop during training, thereby leveraging it as a regularizer reducing
the effect of the Hessian along the optimization trajectory.
Alternatively, SHOT can be utilized as a meta-meta-initializer as is used to
obtain Table \ref{table:randomfeature}. In this approach, the entire model is
pre-trained with SHOT, \ie The outer loss is substituted with $L_{SHOT}$ without utilizing any labeling information. 
Then the model is trained with the original loss function. However, there is a vulnerability to homogeneous
corruption, where the loss goes to zero only if $\theta_t$ and $\theta_r$ produce the same output of all inputs.
As this phenomenon is trivial in the self-supervised learning area, we drew inspiration
from BYOL~\cite{BYOL}. To address this issue, we added a projector to the reference model, while the target remained the same. We also augmented $\mathcal{X}_t^\tau$. After
pre-training with SHOT, we started training by loading the best model with the highest
validation accuracy.
To differentiate between SHOT utilized as a regularizer and SHOT utilized as a meta-meta-initializer, 
we denote them as $\text{SHOT}_r$ and $\text{SHOT}_p$, respectively.

\subsection{SHOT does not require any computation burden}\label{sec:shotcomputation}

%There are some algorithms in meta learning which already assumed linearity in the inner loop. For example, FoMAML and Reptile \cite{maml,Reptile} proposed Hessian-Free GBML algorithm\nj{s}. Both assumed linearity in the inner loop. Also, ANIL \cite{anil} proposed \nj{a} feature reuse concept, which has \nj{room} for translation  to zero distortion in the inner loop. However, none of these researches explicitly argued that \jh{`\textit{GBML implicitly \nj{suppresses} the Hessian in the inner loop}'} is \nj{an} inductive prior, nor they proposed an algorithm that \nj{searches for a small} Hessian.  Rather, our algorithm is similar to ‘SAM’  optimizer \cite{DBLP:journals/corr/abs-2010-01412} \nj{or} natural gradient descent \cite{Riemannian}. Our  algorithm searches \nj{for a} good initialization point regarding its curvature as SAM and natural gradient descent \nj{do}. SHOT finds it in the cost of first-order. Which is notable strong point compared to SAM or natural gradient descent. Although SAM uses first-order computation term, it searches flat minima by iteratively   adding many noises to each point. Natural gradient descent exploits Fisher   metric, which is second-order computation cost.

Several meta-learning algorithms have already assumed linearity in the inner loop. For example, FoMAML and Reptile \cite{maml,Reptile} proposed Hessian-Free GBML algorithms that both assumed linearity in the inner loop. Additionally, ANIL \cite{anil} proposed a feature reuse concept that allows for translation to zero distortion in the inner loop. However, none of these studies explicitly argued that GBML implicitly suppresses the Hessian in the inner loop as an inductive prior, nor did they propose an algorithm that controls the Hessian.
%
Our algorithm is similar to the ‘SAM’ optimizer~\cite{DBLP:journals/corr/abs-2010-01412} or natural gradient descent \cite{Riemannian}. Like SAM and natural gradient descent, our algorithm searches for a good initialization point based on its curvature. However, SHOT finds it without much increasing the computational cost compared to normal gradient descent, which is a notable advantage over SAM or natural gradient descent. Although SAM uses a first-order computation term, it searches for flat minima by iteratively adding noise to each point. Natural gradient descent exploits the Fisher metric, which is a second-order computation cost.

On the other hand, we can make SHOT not give any computation burden. When we set the reference model $\theta_{r}$ to exploit the same number of optimization steps in the inner loop as the baseline model and the target model $\theta_{t}$ exploits one optimization step in the inner loop, because both models share the same initialization point $\theta^0$, \ie $\theta_t^0 = \theta_r^0$\jh{.} $\theta_{t}$ can be obtained by calculating the first optimization step of $\theta_{r}$. Therefore, SHOT does not require any additional backpropagation. What we require is only one more inference at the endpoint  $\theta_{t}^T$ for ${\text{SHOT}_r}$.
Also, even if we set $\theta_{r}$ to have more optimization steps than the baseline model and set $\theta_{t}$ to have the same number of optimization steps as the baseline model, the computation cost at test time is unchanged as it is only used in the training phase.



==> text/5_experiments.tex <==
\section{Experiments}



\textbf{Datasets \ } Our method is evaluated on miniImageNet \citep{miniimagenet},
tieredImageNet \cite{tieredimagenet}, Cars \cite{cars}, and CUB \cite{cub} datasets.
miniImageNet and tieredImageNet are subsets of ImageNet \cite{imagenet} with 100 classes
each and can be considered as general datasets. Cars and CUB are widely used benchmarks for
fine-grained image classification tasks as they contain similar objects with subtle
differences. By conducting experiments on these datasets, we can evaluate the performance of
our method across a range of tasks.



\textbf{Architectures \ } We use 4-Conv from \cite{maml} and ResNet-12 from \cite{metaresnet}
as our backbone architecture. We trained 4-Conv for 30k iterations and ResNet-12 for 10k
iterations.



\textbf{Experimental Setup \ } To ensure a fair comparison, we fine-tuned MAML 
\cite{maml} first, and our baselines outperformed the original paper. We used Adam \cite{adam}
as our optimizer and fixed the outer loop learning rate to $10^{-3}$
and inner loop learning rate to 0.5 for 4-Conv, and $10^{-5}$ and 0.01 for 
ResNet-12. We restricted the total number of steps in the inner loop to 3, 
as argued in \cite{maml}. We set the number of steps to 1 for the target model $\theta_{t}$ and 3 for the reference model $\theta_{r}$ in our SHOT. With this setting, we can exploit
SHOT without any additional computation burden as discussed in Sec~\ref{sec:shotcomputation}.
For 
$\text{SHOT}_r$, we fixed $\lambda$ to 0.1 when we set the 
original model as $\theta_{r}$. For one-step algorithms, we set the number
of optimization steps to 2 for $\theta_{r}$ and 1 for $\theta_{t}$. So 
actual optimization step in inference time is 1, which is the same as the baseline.
We set $\lambda$ for $10^{-6}$ in that case. For the Hessian-Free algorithm FoMAML,
we fine-tuned $\lambda$ to meet the best performance. We set the learning rate
of the outer and inner loops to $10^{-4}$ and 0.01, respectively, for 4-Conv.
To maintain conciseness, we only report the results of $\text{SHOT}_r$ except for the comparison with MAML baseline. We conducted our 
experiments on a single A100 GPU. We implemented our method using torchmeta \cite{torchmeta} library except for the implementation of LEO \cite{LEO}, where we used the official implementation and embeddings.

\input{text/table/LIL_basic.tex}
\input{text/table/Cross_Dataset.tex}

\input{text/table/resnet_lil.tex}

\subsection{Characteristics of SHOT}
\textbf{SHOT Outperforms the Baselines on Benchmarks and Cross-Benchmark Settings \ } 
Our method, SHOT, outperforms the corresponding baseline 
on all benchmarks, as shown in Table \ref{table:4conv_indomain}. Both $\text{SHOT}_r$ and $\text{SHOT}_p$ outperform the baseline, regardless of whether the benchmark is general or fine-grained. Additionally, SHOT generalizes well to cross-benchmark settings, as demonstrated in Table~ \ref{table:4conv_crossdomain},
where it improves the performance of the baseline. Also, we can see that this result is independent
of the backbone architecture, as shown in Table \ref{table:resnet}.


\textbf{SHOT works with Hessian-Free and One-Step algorithms \ } 
As many GBML algorithms 
are based on Hessian-Free algorithms which only exploit gradients and One-Step algorithms which only exploit one step in the
inner loop \cite{maml,Reptile,BOIL,anil}, it is important to show that our method
also works with these algorithms. As shown in Table \ref{table:fo1shot}, our method improves the performance of the baseline on both Hessian-Free and One-Step algorithms.
For One-Step algorithms, we set $\theta_{t}$ as the original model and 
$\theta_{r}$ as the 2-step optimized model. This is practically 
useful since many algorithms exploit only one step in the inner loop. 
Notably, our method is applied only in the training phase, so it has the same inference cost as the baseline. Also, we only used first-order 
optimization for the meta-optimizer to ensure a fair comparison when adding SHOT to FoMAML.
For ANIL~\cite{anil} and BOIL~\cite{BOIL}, we conducted experiments with the same settings from each baseline paper, and we bring the
results from \cite{BOIL} for comparison.
%


\input{text/table/fo_1step}
% As GBML algorithms are inherently unstable, many GBML algorithms use
% regularization techniques to stabilize the training process \cite{imaml, LEO}.
% As SHOT is intended to enforce the implicit prior of GBML during training phase, it
% can be viewed as a regularization technique. To show this, we conducted an experiment
% on LEO \cite{LEO}, which is one of the most popular GBML algorithms that uses a regularization
% in the inner loop. We substituted the regularization term of LEO with SHOT, and the results
% are shown in Table \ref{table:leo}. Although the results are not marginal, SHOT still
% enhances the performance of LEO. Considering LEO works with highly-fine-tuned hyperparameters,
% it is notable that there is still room for improvement. Also, it implies the potential of SHOT
% as a plug-and-play regularization technique for GBML algorithms. As it worked with highly-fine-tuned
% hyperparameters, it can improve the performance more when it is used with other GBML algorithms
% that are not highly-fine-tuned.
%SHOT can act as a regularizer in GBML algorithms. We conducted an experiment on LEO, a popular GBML algorithm that uses regularization in the inner loop, by substituting LEO's regularization term with SHOT. The results, shown in Table \ref{table:leo}, demonstrate that SHOT enhances LEO's performance. This suggests the potential of SHOT as a plug-and-play regularization technique for GBML algorithms, especially those that are not highly-fine-tuned.
% \begin{figure}[t]\label{fig:convergence_speed}
%   \begin{minipage}[c]{0.53\textwidth}
%     \hspace{-7mm}
%     \includegraphics[width=\textwidth]{figure/cossimall.png}
%   \end{minipage}\hfill
%   \begin{minipage}[c]{0.46\textwidth}
%     \caption{In this figure, we present a qualitative analysis of SHOT. We plotted
%     cosine similarity and validation accuracy against training epoch. To ensure a fair
%     comparison, we trained $\text{SHOT}_p$ for 270 epochs. However, for this figure, we trained $\text{SHOT}_r$ for 300 epochs to compare it at a glance. Our results show that SHOT converges much faster than the baseline. Additionally, we observed a strong correlation between
%     cosine similarity and validation accuracy.}
%   \end{minipage}
%   \vspace{-3mm}
% \end{figure}



% \textf{Shot makes faster convergence}. Our method, SHOT, converges faster than the baseline, as shown in figure 
% \ref{fig:convergence_speed}, where we plot the validation 
% accuracy against training epoch. To understand why this 
% happens, we compared the direction from the initial point 
% to the optimized point with each gradient step in the inner loop, 
% as shown in figure \ref{fig:cosine}, and found 
% that overall similarity increases in both cases. Also, it shows that 
% similarity is highly correlated with the validation accuracy.
% SHOT enforces high similarity from the beginning, thereby obtained 
% faster convergence with better generalization. Interesting point is that of all 
% the methods, they have similar dynamics. As seen in Fig. \ref{fig:cosine}, There is a phase where first
% step governs entire inner loop, and other steps are not effective much. After that phase, actual training
% begins. SHOT reduces the time where the model reaches that phase. 

\textbf{SHOT enables faster convergence}. Our method, SHOT, achieves faster convergence
compared to the baseline, as demonstrated in Figure \ref{fig:cosine}, where
we plot the validation accuracy against the training epoch. To understand why this occurs,
we plotted averaged cosine similarity between the overall parameter difference with each inner gradient
step in the inner loop, as shown in Figure \ref{fig:cosine}. We found that overall similarity increases in both cases of with and without SHOT, and the similarity is highly correlated with the validation
accuracy. SHOT enforces high similarity from the beginning, resulting in faster convergence
with better generalization ability. 
% \jh{Interestingly, all methods exhibit similar dynamics, as shown in Figure \ref{fig:cosine}. Initially, there is a phase where the averaged cosine similarity decreases. After this phase, GBML's validation accuracy increases as the averaged cosine similarity increases. We can interpret the success of SHOT as reducing the time it takes for the model to reach this critical phase.}

% Interestingly, all methods exhibit similar dynamics, as
% seen in Figure \ref{fig:cosine}. There is a phase where the averaged cosine similarity reduces. After that phase, GBML's validation accuracy increases with the increase of averaged cosine similarity. We could interpret the success of SHOT that reduces the time it takes for the model to reach that phase.


\textbf{Applying other distance metrics}. We used KL divergence as a distance metric in SHOT, but it is possible to use other
metrics as well. For example, we could use cross-entropy as a distance metric
from a probability perspective, or we could use L2 distance between parameters
as a distance metric. We conducted experiments with different distance metrics, and
for L2 distance we divided the L2 distance by the square root of the number of
parameters to account for the initialization scheme \cite{kumar2017weight}. For the cross-entropy loss, we used the
same $\lambda$ \jh{(balancing term for Eq.~\ref{eq:SHOT})} settings as for KL divergence. The results are shown in Table 
\ref{table:other_distance}. We observed that SHOT outperformed the baseline for every
distance metric. This supports our hypothesis that we can improve performance and dynamics
by suppressing the effect of the Hessian along the optimization trajectory.

% As we used KL divergence as a distance metric in SHOT, it is also feasible to apply other metrics.
% For example, we could use cross-entropy loss as a distance metric as a viewpoint of probability. Also,
% we could use l2 distance between parameters as a distance metric. We conducted experiments with different
% distance metrics. For l2 distance, we devided square root of l2 distance by the number of parameters to meet
% the scale considering initialization scme. For cross-entropy loss, we used the same hyperparameter settings
% as KL divergence. The results are shown in Table \ref{table:other_distance}. We observed that within every 
% distance metric, SHOT have shown better performance than the baseline. This also supports our hypothesis that
% we could improve the performance and dynamics by enforcing the effect of the Hessian along the optimization trajectory.
%

\input{text/table/distance_metric.tex}

==> text/7_Conclusion.tex <==
\section{Conclusion}\label{Section:conclusion}
In this paper, we claim that GBML implicitly suppresses 
the Hessian along the optimization path. We also demonstrate that we 
can improve the performance of GBML by explicitly enforcing this 
implicit prior. To achieve this, we propose a novel method, SHOT 
(Suppressing the Hessian along Optimization Trajectory). Although it deals 
with curvature of the loss surface, it has the same computational order compared to other GBML methods. 
More specifically, it adds a negligible computational overhead  
to the baseline and costs the same at inference time.
We show that SHOT outperforms the baseline and is 
algorithm- and architecture-independent. We believe that 
our method can be applied to other GBML methods in a plug-and-play manner.%that were not included 
%in our experiments. 
%Although it has a slightly higher computational cost 
%than the baseline, it is negligible, and it costs the same at inference time. 
%We hope that our method can be used as a plug-and-play module for other GBML methods.


\section{Acknowledgements}

This work was supported by NRF grant (2021R1A2C3006659) and IITP grants (2021-0-01343, 2022-0-00953), all of which were funded by Korean Government (MSIT).

==> text/table/Hessian_Free.tex <==
\begin{table}[t]
  \caption{Test accuracy \% of 4-conv network on benchmark data sets. The values in parentheses are the number of shots. The better accuracy between the baseline and LIL is bold-faced.}
  \centering
  \begin{center}
    \adjustbox{max width=0.72\textwidth}{%
      \begin{tabular}{c|cc|cc}
        \hline 
        Domain & \multicolumn{2}{c|}{General(Coarse-grained)} & \multicolumn{2}{c}{Specific (Fine-grained)} \\ \hline \hline
        Dataset       & miniImageNet & tieredImageNet & Cars             & Cub              \\ \hline
        FOMAML (1)  & 46.29 $\pm$ 0.94 &   46.96 $\pm$ 0.81  & 47.91 $\pm$ 0.56 &  57.46 $\pm$ 0.21\\
        FOMAML + LIL_p (1) & \textbf{46.81} $\pm$ 0.87 & \textbf{47.86} $\pm$ 0.81 & \textbf{48.45} $\pm$ 0.56 & \textbf{58.01} $\pm$ 1.00\\
        ANIL (1)        & \textbf{50.44} $\pm$ 1.00 & \textbf{50.56} $\pm$ 0.54 & 56.30 $\pm$ 0.76 &        \textbf{63.14} $\pm$ 0.38 \\
        ANIL + LIL_p (1) & 49.91 $\pm$ 0.34 & 50.48 $\pm$ 0.43 & \textbf{56.51} $\pm$ 0.85 & {62.93} $\pm$ 0.03 \\ \hline
        FOMAML (5)       &   62.91	$\pm$ 1.85 & 65.56 $\pm$ 0.89 & 62.75 $\pm$ 1.55 & 71.44 $\pm$ 0.34 \\
        FOMAML + LIL_p (5) &   \textbf{65.05} $\pm$ 1.25 & \textbf{66.37} $\pm$ 0.27 & \textbf{65.69} $\pm$ 3.52 & \textbf{72.52} $\pm$ 0.22\\ 
        ANIL (5)        & 66.34 $\pm$ 0.35 & 69.50 $\pm$ 0.57 & 75.54 $\pm$ 0.22  & \textbf{77.60} $\pm$ 0.12  \\
        ANIL + LIL_p (5) &   \textbf{67.09} $\pm$ 0.59 & \textbf{69.81} $\pm$ 0.17 & \textbf{76.39} $\pm$ 0.02 & {77.19} $\pm$ 0.21 \\\hline
      \end{tabular}
    }
  \end{center}
  \label{table:Hessian_Free}
\end{table}



==> text/table/leo_lil.tex <==
\begin{wraptable}{rt}{7cm}
  \vspace{-5mm}
  \caption{Test accuracy \% of ResNet-12. The values in parentheses are the number of shots. The better accuracy between the baseline and LIL is bold-faced.}
  \centering
  {\tiny
    \begin{center}
      \begin{tabular}{c|ccc}
        \hline
        meta-train    & \multicolumn{3}{c}{miniImageNet}                       \\ \hline \hline
        meta-test     & miniImageNet     & tieredImageNet   & Cars             \\ \hline
        LEO (1)       & 50.63 $\pm$ 1.70 & 54.33 $\pm$ 1.02 & 35.41 $\pm$ 1.01 \\
        LEO + LIL (1)& \textbf{52.72} $\pm$ 0.15 & \textbf{54.66} $\pm$ 0.58 & \textbf{35.75} $\pm$ 0.29 \\ \hline
        LEO (5)       & 71.32 $\pm$ 1.55 & 74.01 $\pm$ 1.69 & 45.75 $\pm$ 0.89 \\
        LEO + LIL (1)& \textbf{72.50} $\pm$ 0.94 & \textbf{75.13} $\pm$ 1.35 & \textbf{48.21} $\pm$ 0.49 \\ \hline
      \end{tabular}
    \end{center}
  }
  \label{table:leo}
\end{wraptable}

